Looped Transformers as Programmable Computers

We present a framework for using transformer networks as universal computers by programming them with specific weights and placing them in a loop. Our input sequence acts as a punchcard, consisting of instructions and memory for data read/writes. We demonstrate that a constant number of encoder layers can emulate basic computing blocks, including embedding edit operations, non-linear functions, function calls, program counters, and conditional branches. Using these building blocks, we emulate a small instruction-set computer. This allows us to map iterative algorithms to programs that can be executed by a looped, 13-layer transformer. We show how this transformer, instructed by its input, can emulate a basic calculator, a basic linear algebra library, and in-context learning algorithms that employ backpropagation. Our work highlights the versatility of the attention mechanism, and demonstrates that even shallow transformers can execute full-fledged, general-purpose programs.

==> Extra.tex <==
\subsection{Read / Write}\label{ss:c2}
We show that data from a location specified in the current command can be read to or written to the scratchpad. 
\begin{lemma}
There exist parameter matrices such that depending on the embedding pointers stored within the scratchpad $\rmS$, the data or command is read from or written to the pointed location to the scratchpad.
\end{lemma}

That is, given the instruction for reading from or writing to location $i$, in the form of the tuple $(b_r, b_w, \vz_i)$, where $b_r, b_w$ are bits representing whether to read or to write, respectively, and $\vz_i$ is the binary ($\pm 1$) vector representation of i, we should be able to do the following (the first column is the scratchpad):
\begin{align*}
\Input = 
     \left[\begin{array}{c|cccc}
        \vv&\vv_2&\dots&\vv_i&\dots\\
     b_r & 0&\dots &0 &\dots\\
        b_w & 0&\dots &0 &\dots\\
        \emb_i &\emb_2&\dots& \emb_i&\dots
    \end{array}\right] \xrightarrow{\text{read when $b_r=1, b_w=0$}}  \left[\begin{array}{c|cccc}
            \vv_i&\vv_2&\dots&\vv_i&\dots\\
                    b_r & 0&\dots &0 &\dots\\
        b_w & 0&\dots &0 &\dots\\
        \emb_i&\emb_2&\dots& \emb_i&\dots\\
    \end{array}\right]
\end{align*}
or
\begin{align*}
\Input = 
     \left[\begin{array}{c|cccc}
     \vv&\vv_2&\dots&\vv_i&\dots\\
              b_r & 0&\dots &0 &\dots\\
        b_w & 0&\dots &0 &\dots\\
        \emb_i &\emb_2&\dots& \emb_i&\dots\\
    \end{array}\right] \xrightarrow{\text{write when $b_w=1, b_r=0$}}  \left[\begin{array}{c|cccc}
    \vv&\vv_2&\dots&\vv&\dots\\
             b_r & 0&\dots &0 &\dots\\
        b_w & 0&\dots &0 &\dots\\
        \emb_i&\emb_2&\dots& \emb_i&\dots\\
    \end{array}\right]
\end{align*}

\paragraph{Proof sketch:}
For doing this operation, we allow some extra rows of zeros in the input as follows:
\begin{align*}
\Input = 
    \left[\begin{array}{c|cccc}
     \vv&\vv_2&\dots&\vv_i&\dots\\
     \zero&\zero&\dots&\zero&\dots\\
              b_r & 0&\dots &0 &\dots\\
        b_w & 0&\dots &0 &\dots\\
        \emb_i &\emb_2&\dots& \emb_i&\dots\\
    \end{array}\right]
\end{align*}

For this, we use an attention head with 
\begin{align*}
    \key =  \query =  \begin{bmatrix}
          \zero &\zero\\
          \zero &\id_{\log(n)} 
         \end{bmatrix} ,
\end{align*}
where the identity matrix has the same dimensions as $\vz_i$. Hence, $\key \Input = [\emb_i\; \emb_2\;\dots\;\emb_i\; \dots]$. Then $\softmax((\key\Input)^\top \query\Input)$ is an $n\times n$ matrix of the following form
\begin{align}
\begin{bmatrix}
    \dfrac{\rve_i +\rve_1}{2} & \rve_2 &\dots& \rve_{i-1} &\dfrac{\rve_i +\rve_1}{2}&\rve_{i+1}&\dots
    \end{bmatrix}  +\epsilon \rmM
\end{align}
where $\|\rmM\|\leq 1$ and $\epsilon$ is as defined in the previous section. We will ignore $\rmM$ in the rest of this proof sketch.

 Looking at \eqref{eq:TF}, $\Input \softmax((\key\Input)^\top \query\Input)$ is as follows:
\begin{align*}
    \Input \softmax((\key\Input)^\top \query\Input) = \left[\begin{array}{c|cccc}
     \frac{\vv + \vv_i}{2}&\vv_2&\dots& \frac{\vv + \vv_i}{2}&\dots\\
     \zero&\zero&\dots&\zero&\dots\\
              b_r/2 & 0&\dots &b_r/2 &\dots\\
        b_w/2 & 0&\dots &b_w/2 &\dots\\
        \emb_i &\emb_2&\dots& \emb_i&\dots\\
    \end{array}\right]
\end{align*}

We set $\out = 2\id$ and 
\begin{align}
\val = \begin{bmatrix}
    \zero &\zero & 0&0&\zero\\
    \id &\zero & 0&0&\zero\\
    \zero &\zero & 1&0&\zero\\
    \zero &\zero & 0&-1&\zero\\
    \zero &\zero & 0&0&\zero
    \end{bmatrix}.
\end{align}

Thus, 
\begin{align*}
    \out \val \Input \softmax((\key\Input)^\top \query\Input) = \left[\begin{array}{c|cccc}
    \zero&\zero&\dots&\zero&\dots\\
     \vv + \vv_i&2\vv_2&\dots& \vv + \vv_i&\dots\\
       b_r & 0&\dots &b_r &\dots\\
   -b_w& 0&\dots &-b_w &\dots\\
    \zero&\zero&\dots&\zero&\dots\\
    \end{array}\right]
\end{align*}
Hence, 
\begin{align*}
    \Input + \out \val \Input \softmax((\key\Input)^\top \query\Input) = \left[\begin{array}{c|cccc}
    \vv&\vv_2&\dots&\vv_i&\dots\\
    \vv + \vv_i&2\vv_2&\dots& \vv + \vv_i&\dots\\
       2b_r & 0&\dots &b_r &\dots\\
  0 & 0&\dots &-b_w &\dots\\
    \zero&\zero&\dots&\zero&\dots\\
    \end{array}\right]
\end{align*}

Let each of the column above be represented as the vector $[\vv_o\;\vv_s\;r\;w\; \vz]$. Then, the feedforward layer of \eqref{eq:TF} can simply implement the following to complete the read / write operations:
\begin{align*}
    \vv_{new} &= \vv_o + \sigma_r(C(r-2) + \vv_s - 2\vv_o) - \sigma_r(C(r-2)  -(\vv_s - 2\vv_o)) \\
    &\quad + \sigma_r(C(-w-1) + \vv_s - 2\vv_o) - \sigma_r(C(-w-1)  -(\vv_s - 2\vv_o)),
\end{align*}
where $C$ is a large enough constant.


However, we have another way of controlling the input, which is by the size of each attention mechanism, that is directly controlled by the dimension $d$ of the embedding.
\begin{lemma}
    Consider an input of the form 
\begin{equation}
    \Input = \begin{bmatrix}
        \vx&\dots&\vx&\vZero\\
        0&\dots&0&0\\
         \vOne-\ve_1&\dots&\vOne-\ve_d&\vOne-\ve_{d+1}\\
        \ve_1&\dots&\ve_d&\ve_{d+1}
    \end{bmatrix}
\end{equation}
where  $\vz = \rve_j \in\R^d$ is an indicator vector and $\rvx\in\R^d$; then there  exists a one layer transformer with $m$ heads such that\AG{What is m here? maybe switch m and d? What each head is doing? How do you choose which function to implement?}  \begin{equation}
    \att(\Input) = \begin{bmatrix}
                 \vx&\dots&\vx&\vZero\\
                 \sigma(\rva_1^\top\vx)&\sigma(\rva_1^\top\vx)&\dots&\sigma(\rva_d^\top\vx)\\
                \vOne-\ve_1&\dots&\vOne-\ve_d&\vOne-\ve_{d+1}\\
        \ve_1&\dots&\ve_d&\ve_{d+1}
     \end{bmatrix}
\end{equation}
\end{lemma}
\begin{proof}
     Let
     \begin{equation}
         \key= \begin{bmatrix}
                \rva_1^\top&0&-C\ve_1^\top&\vZero^\top\\
                \vdots& \vdots& \vdots& \vdots\\
                \rva_d^\top&0&-C\ve_d^\top&\vZero^\top\\
                \vZero^\top&0&\vZero^\top&\vZero^\top
     \end{bmatrix}, \query = \begin{bmatrix}
                \vZero^\top&0&\vZero^\top&\ve_1^\top\\
                \vdots& \vdots&\vdots& \vdots\\
                \vZero^\top&0&\vZero^\top&\ve_{d+1}^\top
     \end{bmatrix}
     \end{equation}
     Hence, \AG{You also need to multiply with $c_i$ and sum them somehow?}
     \begin{equation}
         \key\Input= \begin{bmatrix}
                \rva_1^\top\vx&-C&\dots&-C\\
                -C&\rva_2^\top\vx&\dots&-C\\
                \vdots& \vdots&\vdots& \vdots\\
                -C&-C&\dots&\rva_d^\top\vx\\
                0&0&\dots&0
     \end{bmatrix}, \query\Input = \id_{d+1}
     \end{equation}
     After applying softmax we get,
     \begin{align*}
         \sigma_s((\key\Input)^\top \query\Input) \approx \begin{bmatrix}
                \sigma(\rva_1^\top\vx)&0&\dots&0\\
                0&\sigma(\rva_2^\top\vx)&\dots&0\\
                \vdots& \vdots&\vdots& \vdots\\
                0&0&\dots&\sigma(\rva_d^\top\vx)\\
                *&0&\dots&*
     \end{bmatrix},
     \end{align*}
     for large enough $C$. Next we set 
     \begin{align*}
         \val = \begin{bmatrix}
         0&0&\dots&0 & 0\\
               1&1&\dots&1 &0\\
               0&0&\dots&0 & 0\\
               \vdots&\vdots&\vdots&\vdots & \vdots\\
0&0&\dots&0 & 0
     \end{bmatrix}\query,
     \end{align*}
     thus resulting in 
     \begin{align*}
         \val\Input = \begin{bmatrix}
         0&0&\dots&0 & 0\\
               1&1&\dots&1 &0\\
               0&0&\dots&0 & 0\\
               \vdots&\vdots&\vdots&\vdots & \vdots\\
0&0&\dots&0 & 0
     \end{bmatrix}\query\Input = \begin{bmatrix}
     0&0&\dots&0 & 0\\
               1&1&\dots&1 &0\\
               0&0&\dots&0 & 0\\
               \vdots&\vdots&\vdots&\vdots & \vdots\\
0&0&\dots&0 & 0
     \end{bmatrix}.
     \end{align*}

     Hence, we get
     \begin{align*}
         \val\Input\sigma_s((\key\Input)^\top \query\Input) = \begin{bmatrix}
                 0&0&\dots&0\\
                 \sigma(\rva_1^\top\vx)&\sigma(\rva_1^\top\vx)&\dots&\sigma(\rva_d^\top\vx)\\
                0&0&\dots&0\\
                \vdots& \vdots&\vdots& \vdots\\
                0&0&\dots&0\\
                0&0&\dots&0
     \end{bmatrix},
     \end{align*}
     and 
        \begin{align*}
        \Input + \val\Input\sigma_s((\key\Input)^\top \query\Input) = \begin{bmatrix}
                 \vx&\dots&\vx&\vZero\\
                 \sigma(\rva_1^\top\vx)&\sigma(\rva_1^\top\vx)&\dots&\sigma(\rva_d^\top\vx)\\
                \vOne-\ve_1&\dots&\vOne-\ve_d&\vOne-\ve_{d+1}\\
        \ve_1&\dots&\ve_d&\ve_{d+1}
     \end{bmatrix}.
     \end{align*}
\end{proof}





\subsection{Positional encodings for creating permutation matrices}\label{app:useofPE}
In \eqref{eq:att}, making $\softmax( (\key\Input)^\top \query \Input)$ a permutation matrix can allow different tokens to interact in the feed forward layers. 
As an example, we will first show how we can use the encodings to force the softmax to act as the identity matrix. 

AS we have mentioned, the positional encodings have the following property:
$\emb_i$ is an $\log(n)$ dimensional $\pm 1$ vector which is the binary representation of $i$ with $-1$ in the place of $0$. %
Hence, we have $\emb_i^\top\emb_i = \log(n)$ and each $\emb_i^\top\emb_j < \log(n)$ for $i\neq j$. Let $\key =\query = [\zero \; \id]$ so that $(\key\Input)^\top \query\Input = \embed^\top \embed$. Now, if we apply
the softmax with temperature $\lambda \geq C \log \frac{n}{\epsilon}$ for any big enough constant $C$, we will have for the element $(i, i)$ of the matrix,
\begin{align}
    \bracks{\softmax((\key\Input)^\top \query\Input) }_{i,i}&= 
\dfrac{e^{\lambda \emb_i^\top\emb_i}}{e^{\lambda \emb_i^\top\emb_i} + \sum_{j\neq i} e^{\lambda \emb_i^\top\emb_j} }\\
&= \dfrac{1}{1 + \sum_{j\neq i} e^{\lambda \emb_i^\top\emb_j}/e^{\lambda \emb_i^\top\emb_i} }
\end{align}
Since $\lambda\emb_i^\top\emb_j < \lambda \emb_i^\top\emb_i -\lambda$ for $i\neq j$, we have that 
\begin{align}
    \bracks{\softmax((\key\Input)^\top \query\Input) }_{i,i}&\geq \dfrac{1}{1+ ne^{-\lambda}}\\
    &\geq \dfrac{1}{1+ e^{\log n-\lambda}}\\
    &\geq 1 - \dfrac{e^{\log n-\lambda}}{1+ e^{\log n-\lambda}}\\
    &\geq 1 - e^{\log n-\lambda}
\end{align}
Thus, for  $i\neq j$, $\bracks{\softmax((\key\Input)^\top \query\Input) }_{i,j}\leq  e^{\log n-\lambda}$ and the total error is less than the summation of all the errors, \ie $\mathrm{error} \leq n^2 e^{\log n-\lambda} = e^{3\log n-\lambda}$.

Thus, this matrix is the identity matrix up to error $e^{3\log n-\lambda}$. Similarly, if %



\begin{lemma}\label{lem:sigmoids}
    Consider an input of the form 
\begin{equation}
    \Input = \begin{bmatrix}
        \ve & \zero \\
        \zero & \rvx \\
    \end{bmatrix} \nonumber
\end{equation}
where  $\ve = \rve_j \in\R^N$ is an indicator vector and $\rvx\in\R^d$; then there  exists a one-layer transformer with $m$ heads such that  \begin{equation}
    \att(\Input) = \begin{bmatrix}
        \ve & \zero \\
        \sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji}) & *
    \end{bmatrix} \nonumber
\end{equation}
where $*$ denoted inconsequential values that will be ignored downstream.
\end{lemma}
\begin{lemma}
    Consider an input of the form 
\begin{equation}
    \Input = \begin{bmatrix}
        \rvx & \zero \\
        \zero & \vz \\
    \end{bmatrix}
\end{equation}
where  $\vz = \rve_j \in\R^N$ is an indicator vector and $\rvx\in\R^d$; then there  exists a one-layer transformer with $m$ heads such that  \begin{equation}
    \att(\Input) = \begin{bmatrix}
        \sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji}) & *\\
        \vz & \zero 
    \end{bmatrix},
\end{equation}
where $*$ denoted inconsequential values that will be ignored downstream.
\end{lemma}
\begin{proof}
     Let
     \begin{equation}
         \key^{i} = \begin{bmatrix}
         \zero &\id_d\\
         \zero &\zero 
     \end{bmatrix}, \query^i = \begin{bmatrix}
         -[\rva_{1i} \; \hdots \; \rva_{Ni}] & \zero\\
         \zero &\zero
     \end{bmatrix} , \val^i = \begin{bmatrix}
        \zero &\zero \\
        [c_{1i} \;\hdots \; c_{Ni}]   &\zero
     \end{bmatrix} \nonumber
     \end{equation}

we focus on one head, drop the index $i$ and we have
\begin{align*}
  \val\Input\softmax( (\key\Input)^T(\query\Input) )&= \begin{bmatrix}
        \zero &\zero \\
        [c_{1i} \;\hdots \; c_{Ni}]   &\zero
     \end{bmatrix}\begin{bmatrix}
        \vz & \zero\\
        \zero & \rvx
    \end{bmatrix}\softmax\left(\begin{bmatrix}
        \zero & \rvx\\
        \zero &\zero 
    \end{bmatrix}^T\begin{bmatrix}
        -\rva_{ji} &\zero \\
        \zero &\zero 
    \end{bmatrix}\right)\\
    &= \begin{bmatrix}
        0 &\zero \\
        c_{ji}   &\zero
     \end{bmatrix}\softmax\left(\begin{bmatrix}
         \zero & \zero \\
         -\rvx^T\rva_{ji} &\zero 
     \end{bmatrix}\right)\\
     &=\begin{bmatrix}
        \zero &\zero \\
        c_{ji}   &\zero
     \end{bmatrix}\begin{bmatrix}
          \sigmoid(\rvx^T\rva_{ji})  & * \\
        *& *
     \end{bmatrix}\\
     &= \begin{bmatrix}
         \zero  & \zero\\  
         c_{ji}\sigmoid(\rvx^T\rva_{ji}) & *
     \end{bmatrix}
\end{align*}
After summing over all heads and adding back $\rmX$ through the residual link, we get the desired result.
\end{proof}
In the aforementioned lemma, the desired output is located in a specific sub-block of the output matrix. By utilizing read/write commands, it is possible to copy that function output to any desired location within the output. We show how this can be formally done in \cref{app:functions}.


\begin{lemma}\label{lem:sigmoids_alt}
    Consider an input of the form 
\begin{equation}
    \Input = \begin{bmatrix}
        \vx&\dots&\vx\\
        0&\dots&0&\\
         \vOne-\ve_1&\dots&\vOne-\ve_d\\
        \ve_1&\dots&\ve_d
    \end{bmatrix}
\end{equation}
where  $\ve_i$ is the one hot vector with $1$ in the $i-$th position and $\vx\in$; then there  exists a one layer transformer with 1 head such that
\begin{equation}
    \att(\Input) = \begin{bmatrix}
                 \vx&\dots&\vx\\
                 \sigma(\rva_1^\top\vx)&\dots&\sigma(\rva_d^\top\vx)\\
                \vOne-\ve_1&\dots&\vOne-\ve_d\\
        \ve_1&\dots&\ve_d
     \end{bmatrix}
\end{equation}
\end{lemma}




\begin{proof}
     Let
     \begin{equation}
         \key=  \begin{bmatrix}
                \vZero^\top&0&\vZero^\top&\ve_1^\top\\
                \vdots& \vdots&\vdots& \vdots\\
                \vZero^\top&0&\vZero^\top&\ve_{d}^\top
     \end{bmatrix}, \query =\begin{bmatrix}
                \rva_1^\top&0&-C\ve_1^\top&\vZero^\top\\
                \vdots& \vdots& \vdots& \vdots\\
                \rva_d^\top&0&-C\ve_d^\top&\vZero^\top\\
                \vZero^\top&0&\vZero^\top&\vZero^\top
     \end{bmatrix}
     \end{equation}
     Hence,
     \begin{equation}
         \key\Input= \id_d, \query\Input = \begin{bmatrix}
                \rva_1^\top\vx&-C+\rva_1^\top\vx&\dots&-C+\rva_1^\top\vx\\
                -C+\rva_2^\top\vx&\rva_2^\top\vx&\dots&-C+\rva_2^\top\vx\\
                \vdots& \vdots&\vdots& \vdots\\
                -C+\rva_d^\top\vx&-C+\rva_d^\top\vx&\dots&\rva_d^\top\vx\\
                0&0&\dots&0
     \end{bmatrix}
     \end{equation}
     After applying softmax we get,
     \begin{align*}
         \sigma_s((\key\Input)^\top \query\Input) \approx \begin{bmatrix}
                \sigma(\rva_1^\top\vx)&0&\dots&0\\
                0&\sigma(\rva_2^\top\vx)&\dots&0\\
                \vdots& \vdots&\vdots& \vdots\\
                0&0&\dots&\sigma(\rva_d^\top\vx)\\
                *&0&\dots&*
     \end{bmatrix},
     \end{align*}
     for large enough $C$. Next we set 
     \begin{align*}
         \val = \begin{bmatrix}
         0&0&\dots&0 & 0\\
              1&1&\dots&1 &0\\
              0&0&\dots&0 & 0\\
              \vdots&\vdots&\vdots&\vdots & \vdots\\
0&0&\dots&0 & 0
     \end{bmatrix}
     \end{align*}
     thus resulting in 
     \begin{align*}
         \val\Input = \begin{bmatrix}
         0&0&\dots&0 & 0\\
              1&1&\dots&1 &0\\
              0&0&\dots&0 & 0\\
              \vdots&\vdots&\vdots&\vdots & \vdots\\
0&0&\dots&0 & 0
     \end{bmatrix}%
     \end{align*}

     Hence, we get
     \begin{align*}
         \val\Input\sigma_s((\key\Input)^\top \query\Input) = \begin{bmatrix}
                 0&\dots&0\\
                 \sigma(\rva_1^\top\vx)&\dots&\sigma(\rva_d^\top\vx)\\
                0&\dots&0\\
                \vdots& \vdots&\vdots& \vdots\\
            0&\dots&0\\
                0&\dots&0
     \end{bmatrix},
     \end{align*}
     and 
        \begin{align*}
        \Input + \val\Input\sigma_s((\key\Input)^\top \query\Input) = \begin{bmatrix}
                 \vx&\dots&\vx\\
                 \sigma(\rva_1^\top\vx)&\dots&\sigma(\rva_d^\top\vx)\\
                \vOne-\ve_1&\dots&\vOne-\ve_d\\
        \ve_1&\dots&\ve_d
     \end{bmatrix}.
     \end{align*}
\end{proof}

\begin{corollary}\label{cor:lem_5_alt}
    Consider an input of the form 
\begin{equation}
    \Input = \begin{bmatrix}
        \vx&\dots&\zero\\
        0&\dots&0&\\
         \vOne-\ve_1&\dots&\vOne-\ve_d\\
        \ve_1&\dots&\ve_d
    \end{bmatrix}
\end{equation}
where  $m$ is the number of sigmoids we use and $\ve_i$ is an indicator vector and $\rvx\in\R^d$; then there  exists a 3 layer transformer with 1 head such that
\begin{equation}
    \att(\Input) = \begin{bmatrix}
                 \sum_{i=1}^d\sigma(\rva_1^\top\vx)&\dots&\sum_{i=1}^d\sigma(\rva_1^\top\vx)\\
                \zero&\dots&\zero
     \end{bmatrix}
\end{equation}
\end{corollary}

\begin{proof}
Given the input
    \begin{equation}
    \Input = \begin{bmatrix}
        \vx&\dots&\zero\\
        0&\dots&0&\\
         \vOne-\ve_1&\dots&\vOne-\ve_d\\
        \ve_1&\dots&\ve_d
    \end{bmatrix},
\end{equation}
we set the query and key matrices as follows:
\begin{align*}
    \key = \query = \begin{bmatrix}
        \zero^\top &0&\vOne&\vOne
    \end{bmatrix}.
\end{align*}
Then, we get 
\begin{align*}
    (\key\Input)^\top\query\Input = \begin{bmatrix}
        d&\dots&d\\
        \vdots&\dots&\vdots\\
        d&\dots&d
    \end{bmatrix}.
\end{align*}
Setting the value matrix to 
\begin{align*}
\begin{bmatrix}
    d\id&\zero&\zero&\zero\\
    \zero&\zero&\zero&\zero\\
    \zero&\zero&\zero&\zero\\
    \zero&\zero&\zero&\zero
\end{bmatrix},
\end{align*}
we get 
\begin{align*}
    \val \Input \softmax((\key \Input)^\top \query \Input) = \begin{bmatrix}
        \vx&\dots&\vx\\
        0&\dots&0&\\
        \zero&\dots&\zero\\
        \zero&\dots&\zero
    \end{bmatrix}.
\end{align*}
Hence, the output of the attention layer is:
\begin{align*}
   \Input + \val \Input \softmax((\key \Input)^\top \query \Input) = \begin{bmatrix}
       2\vx&\dots&\vx\\
        0&\dots&0&\\
\vOne-\ve_1&\dots&\vOne-\ve_d\\
        \ve_1&\dots&\ve_d
    \end{bmatrix}.
\end{align*}
Note that using the embeddings in the last rows and a feedforward network can be used to produce the following 

\begin{align*}
\begin{bmatrix}
       \vx&\dots&\vx\\
        0&\dots&0&\\
\vOne-\ve_1&\dots&\vOne-\ve_d\\
        \ve_1&\dots&\ve_d
    \end{bmatrix}.
\end{align*}

Now, passing this into the transformer of \cref{lem:lem_5_alt} will result in 
\begin{equation}
    \att(\Input) = \begin{bmatrix}
                 \vx&\dots&\vx\\
                 \sigma(\rva_1^\top\vx)&\dots&\sigma(\rva_d^\top\vx)\\
                \vOne-\ve_1&\dots&\vOne-\ve_d\\
        \ve_1&\dots&\ve_d
     \end{bmatrix}.
\end{equation}

For the third layer, we set the key and query matrices as follows
\begin{align*}
    \key = \query = \begin{bmatrix}
        \zero^\top &0&\vOne&\vOne
    \end{bmatrix}.
\end{align*}
Then, we get 
\begin{align*}
    (\key\Input)^\top\query\Input = \begin{bmatrix}
        d&\dots&d\\
        \vdots&\dots&\vdots\\
        d&\dots&d
    \end{bmatrix}.
\end{align*}
Setting the value matrix to 
\begin{align*}
\begin{bmatrix}
    \zero&\zero&\zero&\zero\\
    \zero&d&\zero&\zero\\
    \zero&\zero&\zero&\zero\\
    \zero&\zero&\zero&\zero
\end{bmatrix},
\end{align*}
we get 
\begin{align*}
    \val \Input \softmax((\key \Input)^\top \query \Input) = \begin{bmatrix}
        \zero&\dots&\zero\\
\sum_{i=1}^d\sigma(\rva_1^\top\vx)&\dots&\sum_{i=1}^d\sigma(\rva_1^\top\vx)\\
        \zero&\dots&\zero\\
        \zero&\dots&\zero
    \end{bmatrix}.
\end{align*}
Hence, the output of the attention layer is:
\begin{align*}
   \Input + \val \Input \softmax((\key \Input)^\top \query \Input) = \begin{bmatrix}
       \vx&\dots&\vx\\
        \sum_{i=1}^d\sigma(\rva_1^\top\vx)&\dots&\sum_{i=1}^d\sigma(\rva_1^\top\vx)\\
\vOne-\ve_1&\dots&\vOne-\ve_d\\
        \ve_1&\dots&\ve_d
    \end{bmatrix}.
\end{align*}
Finally, the feedforward layers can be used to move the results to the first row.
\end{proof}

==> RelatedWork.tex <==
\begin{itemize}
\item ON THE TURING COMPLETENESS OF MODERN NEURAL NETWORK ARCHITECTURES: 
\begin{itemize}
\item Authors: Jorge Perez, Javier Marinkovi ´ c, Pablo Barcel ´ o
\item Year: 2019
\item Link: \href{https://arxiv.org/pdf/1901.03429.pdf}{Link to paper}
\end{itemize}

\item Attention is all you need: 
\begin{itemize}
    \item Year: 2017 
\item Authors: Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones, Aidan N. Gomez, Lukasz Kaiser, Illia Polosukhin
\item Link: \href{https://arxiv.org/abs/1706.0376}{Link to paper}
\end{itemize}


\item Attention is Turing Complete:
\begin{itemize}
    \item Authors: Jorge Perez, Javier Marinkovi ´ c, Pablo Barcel ´ o
\item Year: 2022
\item Link:  \href{https://www.jmlr.org/papers/volume22/20-302/20-302.pdf}{Link to paper}
\item Uses ideas of the paper above – attention is all you need.
\end{itemize}


\item Inductive biases and Variable creation in self-attention mechanisms: 
\begin{itemize}
    \item Year: 2022
\item Authors: Benjamin L Edelman, Surbhi Goel, Sham Kakade, Cyril Zhang 
\item Link: \href{https://proceedings.mlr.press/v162/edelman22a.html}{Link to paper}
\end{itemize}

\item Statistically Meaningful Approximation: a Case Study on Approximating Turing Machines with Transformers:  
\begin{itemize}
    \item Year: 2021
\item Authors: Colin Wei, Yining Chen, Tengyu Ma
\item Link: \href{https://arxiv.org/pdf/2107.13163.pdf}{Link to paper}
\end{itemize}

\item 


\begin{itemize}
    \item Year: 2020
\item Authors: Satwik Bhattamishra Arkil Patel Navin Goyal
\item Link: \href{https://arxiv.org/pdf/2006.09286.pdf}{Link to paper}
\end{itemize}

\item \href{https://arxiv.org/pdf/1511.08228.pdf}{Neural GPUs}
\item \href{https://arxiv.org/pdf/1410.5401.pdf}{Neural Turing Machines}
\item \href{https://www.nature.com/articles/nature20101.epdf?author_access_token=ImTXBI8aWbYxYQ51Plys8NRgN0jAjWel9jnR3ZoTv0MggmpDmwljGswxVdeocYSurJ3hxupzWuRNeGvvXnoO8o4jTJcnAyhGuZzXJ1GEaD-Z7E6X_a9R-xqJ9TfJWBqz}{NN with dynamic external memory}
\item \href{https://arxiv.org/abs/2211.09066}{Teaching Algorithmic Reasoning}

\item \href{https://openreview.net/forum?id=3m_awcLrg8E}{Token Transformers}
\end{itemize}

==> app_SGD.tex <==
 \begin{figure}
    \centering
    \includegraphics[scale = 0.45]{figures/SGD2.png}
    \caption{Graphical depiction of the building blocks needed to implement SGD. We first read the current data point and use the sigmoids to implement the gradient of the loss. Furthermore, we keep a counter - an integer - that counts the number of points we have iterated through so far and increase it at each iteration. We then check if the counted has iterated all the points; if so we reset the program counter (an embedding) and the counter and continue with the next pass.}
    \label{fig:sgd}
\end{figure}
\begin{theorem}
    Given $\dpoint_i\in\R^d, i=1,\hdots,n-2$  data points and a weight vector $\weight\in\R^d$ as input, there exists an explicit construction of a transformer architecture, of six layers and width $4\log(n) +3d+6$  that simulates SGD over the weight vector. More specifically, for a loss function $f$ it approximately updates the weight vector with gradient steps of the form $\weight - \eta f'(\weight^\top\dpoint_i)\dpoint_i$ and iterates through the points. The error is $\epsilon$ for temperature $\lambda = O(\log(1/\epsilon) + Tn\log(dn))$, if the number of heads used is $m = poly(Tdn)$ for $T$ passes over the $n$ data points.
\end{theorem}
\begin{remark}
    The necessity for $poly(Tn)$ heads is a result of Barron's thorem in \cref{ss:sigmoids}. If we assume that the loss function is a sum of sigmoids the number of heads will be equal to the number of sigmoids we need and the temperature will be $\lambda = O(\log(1/\epsilon) + nTO(\log(dn))$. If we also used masked softmax for everything except for the first two columns (outputs the identity) of the input this can be further improved to $\lambda = O(\log(1/\epsilon) + nTO(\log(d))$.
\end{remark}
\begin{remark}
We can actually encode in the key,query and value weight matrices multiple functions and by having an indicator vector in the input, choose which one we 
 want to use for the gradient steps. Specifically, to apply this, we first linearize the softmax as in \cref{ss:linear} to create the inner product $\weight^\top\dpoint_i$ and then apply the construction presented in \cref{ss:sigmoids}.
\end{remark}

\paragraph{Comparison with prior work.}Closest to this section of our work is the work of \cite{akyurek2022learning}, where the authors prove that constant number of layers is needed to perform one step SGD using decoder only models.
We note here that our analysis for SGD can also be transformed to decoder only models by moving the scratchpad at the end of the input matrix. However, for the rest of the applications decoder only models are somehow restrictive since they don't allow to attend to previous tokens and thus perform operations like ``write back''. The main differences of our work and the work of \citet{akyurek2022learning} are: 1) By using the loop back we don't need proportional to the number of steps of SGD layers  2) we don't use GeLU activations to perform the  inner product between $\weight^\top\dpoint$, but we rather perform the computation inside the attention mechanism, while by forcing the softmax to act as sigmoid we also account for non-linear loss functions 3) we provide an explicit analysis of the error of our result and how it scales depending on the different parameters we choose.
\proof
We consider that the input is of the following form 
\begin{equation}
    \Input = 
\left[\begin{array}{cc|cccccc}
    *&\weight  &*&\hdots& *   \\ 
    \zero &\zero &\dpoint_1 &\hdots &\dpoint_{n-2} \\
     \zero&\zero&\zero &\hdots&\zero   \\
       k & 0 & 0 &\hdots &0\\
      n & 0 & 0 &\hdots &0\\ 
      \mathrm{flag} &0 &0&\hdots &0\\
    \zero&\emb_2 &\emb_3&\hdots &\emb_n  \\
     \emb_\pointer&\zero &\zero&\hdots &\zero  \\
     \emb_2 &\zero &\zero&\hdots &\zero  \\
         \emb_1 & \emb_2& \emb_3 &\hdots &\emb_n   
    \end{array}\right]
    =  \begin{bmatrix}
   *&\weight  &*   \\ 
    \zero &\zero &\dpoints \\
     \zero&\zero&\zero  \\
       k & 0 & \zero\\
      n & 0 & \zero  \\
      \mathrm{flag} &0 &\zero\\
     &\embed_1 &\\
     &\embed_2 &\\
     &\embed_3 &\\
     &\embed_4 &
    \end{bmatrix}
\end{equation}
where $\weight\in\R^{d+2}$ represents the weight vector, $*$ represent arbitrary values, $\dpoints = [\dpoint_1, \hdots, \dpoint_{n-2}]\in\R^{(d+2)\times (n-2)}$ represent the data and $\emb_i$ are the encodings appended to the input;  each $\emb_i$ is of size $ \log(n) +1
$ and it corresponds to the binary representation of the number $i$ with $-1$ in the place of $0$. The extra digit is used for updating the pointer $\emb_\pointer$, as we discussed in \cref{ss:increaseCounter} which shows the column/data point we want to change. This bit is $1$ only for $\emb_\pointer$. Notice that $\emb_i^\top\emb_i = \log(n)$ (or $\log(n)+1$ if it is the pointer) and $\emb_i^\top \emb_j \leq \log(n) -1 $ for all $i\neq j$.

 \textbf{Step 1 - Copy the data point. } After the encodings have been appended to the input we can see that they are in the form of \cref{ss:copy} and thus since we always want to copy in the third block row in which the scratchpad is located (and it is fixed) the input is transformed to 
 \begin{equation}
 \Input_1 =\begin{bmatrix}
   *&\weight  &*   \\ 
    \zero &\zero &\dpoints \\
     \dpoint_\pointer &\zero&\zero  \\
      k & 0 & \zero\\
     n & 0 & \zero \\
     \mathrm{flag} &0 &\zero\\
     &\embed_1 &\\
     &\embed_2 &\\
     &\embed_3 &\\
          &\embed_4 &
    \end{bmatrix}  
\end{equation}
 by using one layer of the transformer architecture. %





\textbf{Step 2 - Create one step of SGD. }
Now we pass this in the next layer which contains an attention like the one described in \cref{ss:sigmoids}. This layer  contains the coefficients that the gradient of the loss has. We also consider that when we are given the weight vector and the data inputs they are both padded with one extra element, which is $-\log(n)$ for the weight and $1$ for the data input. 

So in this layer we will have the following components: $\heads = m$ (depends on the number of sigmoids we want to use to represent the derivative of the loss function
).%
 We ignore the encodings and the last three rows by setting the corresponding rows of the key,query and value matrices to zero for each head $i$; thus the matrices (without the last rows) are %
\begin{equation}
    \key_i = \begin{bmatrix}\zero & \zero &  A_i^\top\\
    \end{bmatrix}, \query_i = \begin{bmatrix}
    \id_{d+1} & \zero &\zero
    \end{bmatrix} 
\end{equation}
and
\begin{equation}
       \out_i = \begin{bmatrix}
   \id_{d+1}\\
        \zero\\
        \zero\\
    
    \end{bmatrix} 
       , \val_i = \begin{bmatrix}
            -\eta c_i\dpoint_\pointer&  \zero & \zero             
       \end{bmatrix}
\end{equation}
\begin{align*}
\Input_1^\top\key_i^\top \query_i\Input_1 & = \parens*{\begin{bmatrix}\zero & \zero &  A_i^\top %
    \end{bmatrix}\begin{bmatrix}
 *&\weight  &*   \\ 
    \zero &\zero &\dpoints \\
     \dpoint_\pointer &\zero&\zero  \\
         \end{bmatrix}}^\top%
\begin{bmatrix}\id_{d+1} &\zero &\zero%
         \end{bmatrix} 
         \begin{bmatrix}
  *&\weight  &*   \\ 
    \zero &\zero &\dpoints \\
     \dpoint_\pointer &\zero&\zero  \\
         \end{bmatrix}\\
         &= \begin{bmatrix}
         A_i\dpoint_\pointer^\top  \\
         \zero \\
         \zero 
         \end{bmatrix}  \begin{bmatrix}
             * &\weight &*\\
         \end{bmatrix}\\
         &= \begin{bmatrix}
         	*&A_i\dpoint_\pointer^\top\weight&*\\
             \zero &\zero &\zero\\
              \zero &\zero &\zero
         \end{bmatrix}
\end{align*}
where $A_i\in\R^{d+1\times d+1}$ is a diagonal matrix containing in all of the diagonal elements the value $a_i$ and $1$ in the last one. Notice that 
$A_i\dpoint_\pointer^\top\weight = a_i\dpoint_\pointer^\top\weight - \log(n)$. Thus, after we apply the softmax we get
\begin{align}
  \softmax(\begin{bmatrix}
         		*&A_i\dpoint_\pointer^\top\weight&*\\
             \zero &\zero &\zero\\
              \zero &\zero &\zero
         \end{bmatrix})  = \begin{bmatrix}
             *&\dfrac{1}{1+ \exp(-a_i\dpoint_\pointer^\top\weight)}&*\\
             *&*&*\\
              *&*&*
         \end{bmatrix}
\end{align}
Notice that the output of the softmax would be $1/(1+\exp(log(n) - log(n) + a_i\dpoint_\pointer^\top\weight)$. Now we have 
\begin{align*}
    \out_i\val_i\Input_1\softmax(\Input_1^\top\key_i^\top \query_i\Input_1) &=  \begin{bmatrix}
        \id_{d+1}\\
        \zero\\
        \zero\\
    \end{bmatrix}
    \begin{bmatrix}
    \zero &\zero &-\eta c_i %
    \end{bmatrix}\begin{bmatrix}
 *&\weight  &*   \\ 
    \zero &\zero &\dpoints \\
     \dpoint_\pointer &\zero&\zero  \\
    \end{bmatrix}\softmax(\Input_1^\top\key_i^\top \query_i\Input_1)\\
    &=\begin{bmatrix}
        \id_{d+1}\\
        \zero\\
        \zero\\
    \end{bmatrix} \begin{bmatrix}
      -\eta c_i\dpoint_\pointer&  \zero & \zero  
    \end{bmatrix}\begin{bmatrix}
                *&\dfrac{1}{1+ \exp(-a_i\dpoint_\pointer^\top\weight)}&*\\
             *&*&*\\
              *&*&*
         \end{bmatrix}\\
          &= \begin{bmatrix}
        \id_{d+1}\\
        \zero\\
        \zero\\
    \end{bmatrix}\begin{bmatrix}
              * & \dfrac{-\eta c_i}{1+\exp(-a_i\dpoint_\pointer^\top\weight)} \dpoint_\pointer  &*
          \end{bmatrix}\\
          &= \begin{bmatrix}
		*&  \dfrac{-\eta c_i}{1+\exp(a_i\dpoint_\pointer^\top\weight)} \dpoint_\pointer &*\\
         \zero  &\zero &\zero\\
         \zero  &\zero &\zero\\
          \end{bmatrix}
\end{align*}
After we sum over all heads and add the residual we get
\begin{equation}
    \Input_2 = \begin{bmatrix}
         *&\weight-\sum_{i=1}^m\dfrac{\eta c_i}{1+\exp(-a_i\dpoint_\pointer^\top\weight)} \dpoint_\pointer &*\\ 
    \zero &\zero &\dpoints \\
     \dpoint_\pointer &\zero&\zero  \\
       k & 0 & \zero\\
      n & 0 & \zero  \\
      \mathrm{flag} &0 &\zero\\
      &\embed_1 &\\
     &\embed_2 &\\
     &\embed_3&\\
     &\embed_4& 
         \end{bmatrix}
\end{equation}
This step requires again one layer.


\textbf{Step 3 - Isolate the counter and increase it. }Consider an extra bit (we don't mention it in the input for simplicity), which is $1$ for the column of $k$ and $0$ everywhere else. Then a \acl{relu} layer can implement the trasformation $k\to k+1$ leaving the rest of the row zero. This can be implement by just one \acl{relu} layer that simply will make the following change $k \to k+1$ and leave the rest of the bits unchanged. And the current input is $\Input_3$. %

\textbf{ Step 4 - If goto. }
Following the analysis presented in \cref{ss:goto} we isolate the program counter $\emb_\pointer$ and implement exactly the following : if $n < k$ then $\emb_\pointer \xleftarrow{} \emb_2$ else $\emb_\pointer \xleftarrow{} \emb_{\pointer +1}$. It is straightforward to see that the input $\Input_3$ is in the correct form to apply \cref{ss:goto}. In the flag the result of $k-n <0$ will be placed. This requires two layers and the new input matrix is $\Input_4$.


\textbf{Step 5 - Reset the counter. }If now the $\mathrm{flag}$ is $1$ we have to reset the counter $k$ to the value $2$ so that it will start counting from the beggining. Again this can be implemented with one \acl{relu} layer that multiplies the flag with $3-n$ and adds it to the counter; thus once the counter is equal to $n+1$ and the $\mathrm{flag}$ is $1$ the counter will get the value of $2$.


\textbf{Analysis of the error. } The proof so far doesn't contain the error that results from 1) the use of the copy operation in step one and 2) the approximation error of the function $f'$.

From \cref{app:lexigerror} \jnote{dead ref} we know that instead of the matrix $\Input_1$, we have a matrix $\Input_1^{'}$ such that 
\begin{equation}
  \Input_1^{'} = \Input_1 + \varepsilon  \rmM
\end{equation}
where $\norm{\rmM}\leq 1$ and $\varepsilon \leq  e^{3\log n-\lambda} $ is a parameter we can control through the temperature $\lambda$ of the softmax (see \cref{app:useofPE})\footnote{If we consider masked attention for all the rows except for the first one in which the copy operation is done we will get the error only on the first column.}. Thus, we have to 
find the difference of 
\begin{align}
    \att(\Input_1) &= \Input_1 + \sum_{i=1}^m \out_i\val_i\Input_1\softmax(\Input_1^\top\key_i^\top \query_i\Input_1)\\
    \att(\Input_1 +\varepsilon\rmM) &= \Input_1 +\varepsilon\rmM + \sum_{i=1}^m \out_i\val_i(\Input_1 +\varepsilon\rmM) \softmax((\Input_1 + \varepsilon\rmM)^\top\key_i^\top \query_i(\Input_1 + \varepsilon\rmM))
\end{align}
We define
\begin{equation}
    E := \norm{\Input_1  - \Input_1 - \varepsilon\rmM}\leq \varepsilon,
\end{equation}
and 
\begin{align}
    F &:= \norm{\sum_{i=1}^m \out_i\val_i\varepsilon\rmM\softmax((\Input_1 + \varepsilon\rmM)^\top\key_i^\top \query_i(\Input_1 + \varepsilon\rmM))}\\
    &\leq  \varepsilon\sum_{i=1}^m \norm{\out_i\val_i\softmax((\Input_1 + \varepsilon\rmM)^\top\key_i^\top \query_i(\Input_1 + \varepsilon\rmM))}\\
    &\leq \varepsilon \sum_{i=1}^m n C(d+1)\\
    &\leq \varepsilon C m n(d+1)\\
    &\leq \varepsilon O(mnd)
\end{align}
Finally, 
\begin{align}
    G &:= \norm{\sum_{i=1}^m \out_i\val_i\Input_1\parens*{\softmax(\Input_1^\top\key_i^\top \query_i\Input_1) -\softmax((\Input_1 + \varepsilon\rmM)^\top\key_i^\top \query_i(\Input_1 + \varepsilon\rmM)) } }\\
    &\leq  C (d+1) \sum_{i=1}^m\norm{\softmax(\Input_1^\top\key_i^\top \query_i\Input_1) -\softmax((\Input_1 + \varepsilon\rmM)^\top\key_i^\top \query_i(\Input_1 + \varepsilon\rmM))}\\
    &\leq C (d+1) \sum_{i=1}^m\norm{\Input_1^\top\key_i^\top \query_i\Input_1 - (\Input_1 + \varepsilon\rmM)^\top\key_i^\top \query_i(\Input_1 + \varepsilon\rmM))}\\
    &\leq C (d+1) \sum_{i=1}^m \norm{\varepsilon\rmM^\top\key_i^\top \query_i\Input_1 + \Input_1\key_i^\top \query_i\varepsilon\rmM + \varepsilon^2\rmM^\top\key_i^\top \query_i\rmM}\\
    &\leq C (d+1) \sum_{i=1}^m2\varepsilon \norm{\Input_1}a_i(d+1) + \varepsilon^2a_i(d+1)\\
    &\leq \varepsilon O(d^3 n m a_i)\\
    &\leq \varepsilon O(d^3 n m^{3/2}\log m)
\end{align}
where $C$ is a constant that depends on the bound of $c_i's$ , $\norm{\Input_1}$ depends on the bound of the input, \ie the set $B$ that the loss function is defined and $a_i = m^{1/2} \log m$ (see \cref{ss:sigmoids}).
In the third step the error is zero, since the increase is exact and the encodings are stay intact during the previous steps. Thus after one step the error is $E+F+G = \varepsilon O(d^3nm^{3/2}\log m)$ and
after $n$ steps the error will be 
of the order $\varepsilon O((d^3nm^{3/2}\log m)^n)$. Hence, to achieve an error less than $\epsilon$, we require the temperature to be 
$\lambda = O (log(1/\epsilon) + n\log(dnm\log m))$.

\begin{remark}
    If we want to run $T$ passes over the data we will have to also encounter for this  and thus $\lambda$ would be $ O (log(1/\epsilon) + Tn\log(dnm\log m))$ to achieve an $\epsilon$ error.
\end{remark}
\begin{remark}
    In this analysis we didn't encounter for the error of the approximation of the function. This error would actually accumulate and be of the order $nT/\sqrt{m}$, since each pass updates the weight vector with error $O(1/\sqrt{m})$. Thus, if  we have $m = O(n^2T^2/\epsilon^2)$ heads we can again achieve $\epsilon$  approximation error. However, if the loss function is a linear combination of sigmoids this error is exactly zero, while also the coefficients $a_i$ don't need to be of the order $m\log m$, since this results from using \cref{th:Barron}. 
\end{remark}
 


==> one_instruction.tex <==
The operations described in the previous section enable us to implement the one instruction set computer, which says that any machine able to execute code consisting of One-Instruction Set Computer instructions is a universal computer. OISC instructions take the following form:
\begin{algorithm}
\caption{One-Instruction Set Computer instruction}\label{alg:cap}
\begin{algorithmic}[1]
    \Statex{\textbf{Inputs}: a, b, c}
    \State {Mem[b] = Mem[b] - Mem[a]}   
    \If {Mem[b] < 0} \State{goto c}
    \Else { goto next instruction}
    \EndIf
\end{algorithmic}
\end{algorithm}

For our case, we will represent this instruction simply as the vector $[\vz_a^\top\;\vz_b^\top\;\vz_c^\top]$.
\subsection{Step 1}
For the step Mem[b] = Mem[b] - Mem[a], we need to 
\begin{enumerate}
    \item Copy Mem[b] and Mem[a] into the scratchpad. This can be done using the pointers $z_b$ and $z_a$, and the operation in Section 4.2.
    \item Compute Mem[b] - Mem[a]. This can be done in a single feed forward layer operations.
    \item Copy Mem[b] - Mem[a] back to location b. This can be done using the $z_b$ pointer and the operation described in Section 4.3.
\end{enumerate}

\subsection{Step 2 and 3}
For the step `if ... goto... else',
\begin{enumerate}
    \item We increment the current instruction pointer $\vz_p$ to get $\vz_{p+1}$ using the operator described in Subsection 4.4.
    \item We compute whether the condition is true using the operation described in Section 4.6.
    \item We update the current pointer using the conditional update described in Section 4.5.
\end{enumerate}

==> table.tex <==
\renewcommand{\arraystretch}{1.5}

\begin{center}
\begin{tabular}{ |c|c|c|c| } 
\hline
\textbf{Applications} & Layers & Width &Heads\\
\hline
SGD & $3$ &$3(\log(n) +d+1)$&$m$\\
\hline
OSIC& $9$& $9\log(n)+1$& 2\\
\hline
Linear Algebra & &&\\
\hline
Calculator& & & \\
\hline
\end{tabular}
\end{center}


\newlength{\brickwidth}
\newlength{\brickheight}
\newlength{\brickdia}
\newlength{\brickdiaheight}
\newlength{\brickmultipliedx}
\newlength{\brickmultipliedy}
\newlength{\halfbrickwidth}
\setlength{\brickheight}{9.6mm}
\setlength{\brickwidth}{8mm}
\setlength{\brickdia}{2.8mm}
\setlength{\brickdiaheight}{1mm}
\setlength{\halfbrickwidth}{0.5\brickwidth}

\newcommand{\startpos}[3]{($(0,#3\brickheight)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)$)}
\newcommand{\startposplusheight}[3]{($(0,#3\brickheight)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)+(0mm,\brickheight)$)}
\newcommand{\pinposone}[5]{($(0,#3\brickheight)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)+(7:#4*\brickwidth)+(138:#5*\halfbrickwidth)+(-0.6\brickwidth,-\halfbrickwidth)+(-0.05\brickwidth,1.35\brickheight)$)}
\newcommand{\pinpostwo}[5]{($(0,#3\brickheight)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)+(7:#4*\brickwidth)+(138:#5*\halfbrickwidth)+(-0.6\brickwidth,-\halfbrickwidth)+(0.3\brickwidth,1.35\brickheight)$)}


\newcommand{\pins}[6]{%
\foreach \i in {#1,...,1} {
  \foreach \j in {#2,...,1} {
    \pin{\pinposone{#4}{#5}{#6}{\i}{\j}}{\pinpostwo{#4}{#5}{#6}{\i}{\j}}{#3}
  }
}
}

\newcommand{\brick}[7]{%
\setlength{\brickmultipliedx}{#1\brickwidth}
\setlength{\brickmultipliedy}{#2\brickwidth}
\filldraw[fill=#3,draw=black,thick] \startpos{#4}{#5}{#6} -- ++(7:\brickmultipliedx) -- ++(0mm,\brickheight) -- ++(138:0.5\brickmultipliedy) -- ++(187:\brickmultipliedx) -- ++(0mm,-\brickheight) -- cycle;
\draw[black,thick] \startpos{#4}{#5}{#6} -- ++(0mm,\brickheight) -- ++(138:0.5\brickmultipliedy);
\node at \startpos{#4}{#5}{#6} {#7};
\draw[black,thick] \startposplusheight{#4}{#5}{#6} -- ++(7:\brickmultipliedx) -- ++(138:0.5\brickmultipliedy);
}

\newcommand{\pin}[3]{%
\draw[thick] #2 ++(\brickdia,-1.2\brickdiaheight) arc(0:-180:{\brickdia} and {\brickdiaheight});
\filldraw[fill=#3,draw=black,thick] #1 -- ++(0mm,-1.2\brickdiaheight) ++(2\brickdia,0mm) -- ++(0mm,1.2\brickdiaheight) -- cycle;
\filldraw[fill=#3,draw=black,thick] #2 ++ (0mm,0.2\brickdiaheight) ellipse[x radius=\brickdia, y radius=\brickdiaheight];
}

\definecolor{myred}{rgb}{0.8,0.45,0.5}
\definecolor{myblue}{rgb}{0.3,0.6,0.9}
\definecolor{myyellow}{rgb}{1,1,0.4}


\newcommand{\LegoDecomposition}{%
\begin{tikzpicture}

  \brick{4}{2}{myblue}{1}{-1}{-1}
  \pins{4}{2}{myblue}{1}{-1}{-1}
  
  \brick{2}{2}{myblue}{2}{0}{0}
  \pins{2}{2}{myblue}{2}{0}{0}

  \brick{1}{6}{myblue}{0}{0}{-1}
  \pins{1}{6}{myblue}{0}{0}{-1}

  \brick{1}{3}{myblue}{0}{2}{0}
  \pins{1}{3}{myblue}{0}{2}{0}
  
  \brick{2}{2}{myred}{0}{0}{0}
    
    \brick{2}{1}{myred}{1}{1}{1}
    \pins{2}{1}{myred}{1}{1}{1}
        
    \brick{1}{3}{myred}{0}{1}{1}
    \pins{1}{3}{myred}{0}{1}{1}
  
  \pins{2}{1}{myred}{0}{0}{0}

  \pins{2}{1}{myblue}{2}{0}{0}
  \pins{4}{1}{myblue}{1}{-1}{-1}
\end{tikzpicture}}


\newcommand{\LegoSingleton}{%
\begin{tikzpicture}


  \brick{3}{1}{myblue}{-1}{0}{-1}
  \brick{1}{2}{myblue}{1}{-1}{0}
  \brick{1}{1}{myred}{0}{0}{0}
  \brick{2}{1}{myblue}{-2}{0}{0}

  \pins{1}{2}{myblue}{1}{-1}{0}
  \pins{1}{1}{myred}{0}{0}{0}
  \pins{2}{1}{myblue}{-2}{0}{0}
  
\end{tikzpicture}
}

\newcommand{\LegoExample}{%

\begin{tikzpicture}
  \brick{3}{1}{myyellow}{6}{0}{0}
  \brick{4}{2}{myblue}{2}{0}{0}
  \pins{4}{2}{myblue}{2}{0}{0}
  
  \brick{2}{4}{myred}{0}{0}{0}
  \brick{2}{4}{myred}{0}{1}{1}
  
  \pins{3}{1}{myyellow}{6}{0}{0}
  
  \pins{2}{1}{myred}{0}{0}{0}
  \pins{2}{4}{myred}{0}{1}{1}
  
  \end{tikzpicture}
  
}
\%begin{tikzpicture}


==> temp.tex <==



\paragraph{Stochastic Gradient Descent.} In this section we show how we can implement multiple passes of SGD using our unified framework. The program provided in \cref{alg:sgd} iterates through the $n$ data points that the user gives and cycles back to the first point after one pass is completed.  The commands we provide below construct a flexible template in which the user can choose 1) the step-size $\eta$ and 2) the loss function through the indicator vector $\ve$ from a set of predefined functions.

\begin{lemma}
Let $\eps > 0$, there exists a transformer with 13 layers, $poly(n_dT)$ heads and dimensionality $O(\log(n_d)+d)$ that uses the Unified Attention Based Computer framework in \cref{sec:fleq} to implement $T$ iterations of SGD on a weight vector $\weight\in\R^d$, over a set of $n_d$ data points $\dpoint_i\in\R^d$, $i=1,\hdots,n_d$ with error up to $\eps$. The step size is given as a parameter to the program, while the loss function can be chosen to be any function of a predefined set of functions $\mathcal{F} = \{f_i\}_{i=1}^N$. 
\end{lemma}
\begin{remark}
The error is controlled by three parameters: the temperature $\lambda$, the constants used in the proof of \cref{lem:matrixmul} and the approximation of the functions $f_i$. Specifically, 
    the necessity for $poly(Tn_d)$ heads is a result of Barron's theorem (\cref{th:Barron}) applied in \cref{lem:sigmoids},  in order to ensure control over the approximation error. If it is assumed that the loss function is a sum of sigmoids, the number of heads will be equal to the number of sigmoids required, and there will be no error associated with this aspect of the construction.
\end{remark}
Closest to this section of our work is the work of \cite{akyurek2022learning}, where the authors prove that constant number of layers is needed to perform one step SGD using decoder only models.
The main differences of our work and the work of \citet{akyurek2022learning} are the following. Firstly, by using the loop back we don't need proportional to the number of steps of SGD layers, instead it is fixed and equal to eleven independently of the number of iterations. Furthermore, our implementation doesn't make use of GeLU activations to perform the  inner product between $\weight^\top\dpoint$, but we rather perform the computation inside the attention mechanism using our  result for matrix multiplication (\cref{lem:matrixmul}); while by forcing the softmax to act as sigmoid we also account for non-linear loss functions. %


\begin{algorithm}[H]
        \caption{Program to simulate SGD using our Unified Attention Based Computer}
        \begin{algorithmic}[1]
            \Require $\texttt{mem}[w]=\weight$, $\texttt{mem}[\eta]=\eta$. 
            \Comment{Location of the weight and  step-size.}
            \Require $\texttt{mem}[z] = \ve.$\Comment{Indicator for the choice of  loss function}
            \Require  $\texttt{mem}[a_0+i-1]=\dpoint_i$, $i=1,\hdots,n_d$. \Comment{Location of the data points.}
            \Require  $\emb_{a_*}=a_0$. \Comment{$\emb_{a_*}$ is a pointer to the first data. }%
            \Require  $\emb_{\pointer} = \text{instr}_1$. \Comment{Program Counter points to first instruction. }
            \Require $\texttt{mem}[q] = 1$, $\texttt{mem}[p]=0$, $\texttt{mem}[z] = n$. \Comment{Constants.}
            \Require %
            $\texttt{mem}[j] =-n_d$.\Comment{Within epoch iteration counter initialized to $-n$.}
            \Require %
            $\texttt{mem}[k] =-T$.\Comment{Epoch counter initialized to $-T$.}
            \vspace{0.5ex}
            \State ( $\text{instr}_1$) \quad $\texttt{mem}[temp] = f_{\text{mul}} ( \texttt{mem}[\emb_{a_*}],\texttt{mem}[w])$. \Comment{Inner product: $\weight^\top \dpoint_i$.}
            \vspace{0.2em}
            \State $\texttt{mem}[temp] = f_{\text{sigmoid}}(\texttt{mem}[z],\texttt{mem}[temp])$. \Comment{Apply sigmoids. }
           \vspace{0.2em}
           \State ( $\text{instr}_3$) \quad $\texttt{mem}[temp] = f_{\text{mul}}( \texttt{mem}[\emb_{a_*}],\texttt{mem}[temp])$. \Comment{Multiply with the data point $\dpoint_i$. }
           \vspace{0.2em}
                \State $\texttt{mem}[temp] = f_{\text{mul}}(\texttt{mem}[temp],\texttt{mem}[\eta])$. \Comment{Multiply with the step-size.}
            \vspace{0.2em}
             \State $\texttt{mem}[w] = f_{\text{sub}}(\texttt{mem}[w],\texttt{mem}[temp])$. \Comment{Subtract from $\weight$ one gradient step.}
             \vspace{0.2em}
        \State $\texttt{mem}[\text{instr}_1] = f_{\text{incr\_pointer}}(\texttt{mem}[\text{instr}_1]).$\Comment{Increment pointer.}
        \vspace{0.2em}
        \State $\texttt{mem}[\text{instr}_3] = f_{\text{incr\_pointer}}(\texttt{mem}[\text{instr}_3]).$ \Comment{Increment pointer.}
        \vspace{0.2em}
        \State $\texttt{mem}[j] = f_{\text{add}} (\texttt{mem}[j], \texttt{mem}[q])$.\Comment{Increment within epoch iteration counter by 1.}
        \vspace{0.2em}
        \State if $\texttt{mem}[j]\leq 0$ goto 1. \Comment{Cycle back to the first data point.}
        \vspace{0.2em}
        \State $\texttt{mem}[j] = -n_d.$ \Comment{Reset counter.}
        \vspace{0.2em}
        \State $\texttt{mem}[\text{instr}_1] = f_{\text{reset\_pointer}}(\texttt{mem}[\text{instr}_1], a_0).$ \Comment{Reset pointer.}
        \vspace{0.2em}
        \State $\texttt{mem}[\text{instr}_3] = f_{\text{reset\_pointer}}(\texttt{mem}[\text{instr}_3], a_0).$ \Comment{Reset pointer.}
        \vspace{0.2em}
        \State $\texttt{mem}[k] = f_{\text{add}} (\texttt{mem}[k], \texttt{mem}[q])$.\Comment{Increment epoch counter by 1.}
        \vspace{0.2em}
        \State if $\texttt{mem}[k]\leq 0$ goto 1. \Comment{Cycle back to the first data point.}
        \vspace{0.2em}
        \State EOF. \Comment{End of File command.}
        \end{algorithmic}\label{alg:sgd}
    \end{algorithm}

\cref{alg:sgd} implements the following gradient update: $\weight_{t+1} = \weight_t -\eta\sum_{i=1}^{n_d} f'(\weight^\top\dpoint_i)\dpoint_i$, where $\dpoint_i$ is the $i-$th data point with its label, $f$ is the loss function and $\eta$ is the step-size.  In the attention mechanism, the derivative of the loss $f'$ is encoded as a sum of sigmoids using \cref{lem:sigmoids}. 

The following will detail the essential procedures for implementing the Stochastic Gradient Descent algorithm. We employ two pointers, namely $\emb_{a_*}$ and $\emb_{\pointer}$, in our algorithm. The first one, referred to as  program counter,   is used to iterate through the commands; after one pass over all data points is completed the program counter is reset to the first instruction (line 14), until $T$ full passes have been completed. The second one, referred to as data pointer, iterates through the data points one by one. The increment of the pointer $\emb_{a_*}$ needs to occur in both instructions 1 and 3, as to in the next iteration they have been updated  from $\text{instr}_i(\emb_{a_*},w,temp) \to \text{instr}_i(\emb_{a_*}+1,w,temp)$, $i=1,3$.

Notice that the functions $f_{\text{incr\_pointer}}$ and $f_{\text{reset\_pointer}}$ can be directly implemented using \cref{app:increase}.




\begin{algorithm}[H]
\caption{Back-Propagation}\label{alg:backprop}
\begin{algorithmic}[1]
\Statex {Loss function: $J(x)= \frac{1}{2}x^2$}
 \Statex{ Input: $\weights_1\in\R^{m\times d}$, $\bias_1\in \R^m$, $\weights_2\in\R^{m\times 1}$, $\bias_2\in\R$ $\dpoint\in\R^d$, $y\in\R$}
 \State Compute $\vz = \weights_1 \dpoint +\bias_1$.
 \State Compute $ \va = \sigma(\vz)$.
 \State Compute $o = \weights_2\va +\bias_2$.
 \State Compute $\delta_2 = (o-y)$.
 \State Compute $\delta_1 =  \sigma'(\vz) \odot\weights_2 (o-y) $.
 \State Compute $\frac{\partial J}{\partial\weights_2} = \delta_2 \va^\top$.
 \State Compute $\frac{\partial J}{\partial\bias_2} = \delta_2$.
 \State Compute $\frac{\partial J}{\partial\weights_1} = \delta_1\dpoint^\top$.
 \State Compute $\frac{\partial J}{\partial\bias_1} = \delta_1$.
\end{algorithmic}
\end{algorithm}
\paragraph{Back-Propagation.} 
 Back-propagation (\cref{alg:backprop}) consists of the following steps: 1) Feed forward the input through the network to calculate the predicted output 2) Calculate the error between the predicted output and the true output 3) Propagate the error backwards through the network, adjusting the weights of the network 4) Repeat steps 1 to 3 for multiple rounds. 
 
We implement steps 1-3 through our unified template; we omit the last step since it can be done by adding an if ... goto command at the end similar to lines 13-14 in \cref{alg:sgd}. The algorithm is given below in \cref{alg:backprop}; two remarks about this implementation are in order.  Line 5 in the algorithm of  Back-propagation (\cref{alg:backprop}) requires an element-wise multiplication. However, the current constructions do not support this operation. To overcome this limitation, the vectors $\vz$ and $\rmW_2$ must be transposed and saved in a new location, then iterated through using a pointer. Additionally, it should be noted that the derivative of the activation function, $\sigma'$, may contain errors as it is approximated as a sum of sigmoids.


\begin{lemma}
There exists a transformer with 13 layers, $poly(mT)$ heads and dimensionality $O(\log(m)+d)$ that uses the Unified Attention Based Computer framework in Section~\ref{sec:fleq} to approximately implement $T$ iterations of Back-propagation algorithm  on a two layer neural network with hidden size $m$.
\end{lemma}
\begin{algorithm}[H]
        \caption{Program to simulate Back-Propagation for two layer Neural Networks}
        \begin{algorithmic}[1]
            \Require $\texttt{mem}[W_1]=\weights_1$,  $\texttt{mem}[W_2]=\weights_2$. \Comment{Weight matrices.}
            \vspace{0.2em}
            \Require  $\texttt{mem}[b_1] = \bias_1$, $\texttt{mem}[b_2] = \bias_2$. \Comment{Biases.}
            \vspace{0.2em}
            \Require $\texttt{mem}[x] = \dpoint$, $\texttt{mem}[y] = y$. \Comment{Data.}
            \vspace{0.2em}
            \Require $\texttt{mem}[q] = 1$, $\texttt{mem}[p]=0$, $\texttt{mem}[r] =-1$, $\texttt{mem}[m] = m$. \Comment{Constants.}
            \vspace{0.2em}
            \Require %
            $\texttt{mem}[k] =1$.\Comment{Iteration counter,  $k:=1$.}
            \vspace{0.2em}
            \Require $\emb_{z} = z_{\textsc{T}}^1$. 
            \Comment{Pointer for $z$.}
            \vspace{0.2em}
            \Require $\emb_{\delta} = \delta_{1,\textsc{T}}^1$. \Comment{Pointer for $\delta_1$.}
            \vspace{0.2em}
            \Require $\emb_{\pointer} = \text{instr1}.$ \Comment{Program Counter shows at the first line of code.}
            \vspace{0.5ex}
            \State ( $\text{instr}_1$) $\texttt{mem}[temp] = f_{\text{trans}} (\texttt{mem}[W_1], \texttt{mem}[p])$. 
            \Comment{Create $\weights_1^\top$.}
            \vspace{0.2em}
            \State $\texttt{mem}[z] = f_{\text{mul}} (\texttt{mem}[temp], \texttt{mem}[x])$. 
            \Comment{Multiply: $\weights_1 \dpoint$.}
            \vspace{0.2em}
           \State $\texttt{mem}[z] = f_{\text{add}}(\texttt{mem}[z],\texttt{mem}[b_1])$. \Comment{Add the bias: Compute $\vz$. }
           \vspace{0.2em}
           \State $\texttt{mem}[a] = f_{\text{relu}}(\texttt{mem}[z],\texttt{mem}[q])$. \Comment{Compute $\va = \relu(\vz)$. }
           \vspace{0.2em}
           \State $\texttt{mem}[temp] = f_{\text{trans}} (\texttt{mem}[W_2], \texttt{mem}[p])$. 
            \Comment{Create $\weights_2^\top$.}
            \vspace{0.2em}
            \State $\texttt{mem}[o] = f_{\text{mul}}(\texttt{mem}[temp],\texttt{mem}[a])$. \Comment{Multiply: $\weights_2\va$.}
            \vspace{0.2em}
            \State $\texttt{mem}[o] = f_{\text{add}}(\texttt{mem}[o],\texttt{mem}[b_2])$. \Comment{Add bias: Compute $o$.}
            \vspace{0.2em}
             \State $\texttt{mem}[\delta_2] = f_{\text{sub}}(\texttt{mem}[o],\texttt{mem}[y])$. \Comment{Compute $\delta_2$.}
            \vspace{0.2em}
             \State $\texttt{mem}[\delta_1] = f_{\text{mul}}(\texttt{mem}[W_2],\texttt{mem}[\delta_2])$. \Comment{Multiply $\weights_2\delta_2$.}
             \vspace{0.2em}
             \State $\texttt{mem}[flag] = f_{\text{sub}}(\texttt{mem}[k],\texttt{mem}[m])$. \Comment{Create $k-m$.}
             \vspace{0.2em}
              \State $ \texttt{mem}[\emb_z] = f_{\text{trans}}(\texttt{mem}[z],\texttt{mem}[p])$. \Comment{Store $\vz$ to consecutive memory cells.}
             \vspace{0.2em}
             \State  $ \texttt{mem}[\emb_\delta] = f_{\text{trans}}(\texttt{mem}[\delta_1],\texttt{mem}[p])$. \Comment{Store $\delta_1$ to consecutive memory cells.}
             \vspace{0.6em}
             \State if $\texttt{mem}[flag]\leq 0$ goto 20.\Comment{If we iterated all the elements goto next command. }
             \vspace{0.2em}
            
             \State ( $\text{instr}_{14}$) $\texttt{mem}[temp'] = f_{\text{sigmoids}}(\texttt{mem}[p],\texttt{mem}[\emb_z])$. \Comment{Create $\sigma'(z_i)$.}
             \vspace{0.2em}
             \State ( $\text{instr}_{15}$) $\texttt{mem}[\emb_\delta] = f_{\text{mul}}(\texttt{mem}[temp'],\texttt{mem}[\emb_\delta])$. \Comment{Create $\sigma'(z_i)(\weights_2)_i(o-y)$.}
             \vspace{0.2em}
             \State $\texttt{mem}[\text{instr}_{14} ]= f_{\text{incr\_pointer}}(\texttt{mem}[\text{instr}_{14}])$. \Comment{Point to next element of $z$.}
             \vspace{0.2em}
             \State $\texttt{mem}[\text{instr}_{15} ]= f_{\text{incr\_pointer}}(\texttt{mem}[\text{instr}_{15}])$. \Comment{Point to next element of $\delta_1$.}
             \vspace{0.2em}
        \State $\texttt{mem}[k] = f_{\text{add}} (\texttt{mem}[k], \texttt{mem}[q])$.\Comment{Increment counter, $k:=k+1$.}
        \vspace{0.2em}

        \State If $\texttt{mem}[p]\leq 0$ goto 13.\Comment{Loop back.}
        \vspace{0.2em}
        
        \State $\texttt{mem}[\text{instr}_1] = f_{\text{reset\_pointer}}(\texttt{mem}[\text{instr}_{14}], z^1_\top)$. \Comment{Reset pointer.}
        \vspace{0.2em}
        \State $\texttt{mem}[\text{instr}_{15}] = f_{\text{reset\_pointer}}(\texttt{mem}[\text{instr}_{15}], \delta_{1,\top}^1)$. \Comment{Reset pointer.}
        \vspace{0.2em}
        \State  $\texttt{mem}[grad\_W_2] =f_{\text{mul}}(\texttt{mem}[\delta_2],\texttt{mem}[a])$. \Comment{Create $\frac{\partial J}{\partial \rmW_2}$.}
        \vspace{0.2em}
        \State  $\texttt{mem}[grad\_b_2] =f_{\text{mul}}(\texttt{mem}[\delta_2],\texttt{mem}[q])$. \Comment{Create $\frac{\partial J}{\partial \rvb_2}$.}
        \vspace{0.2em}
         \State  $\texttt{mem}[grad\_W_1] =f_{\text{mul}}(\texttt{mem}[\delta_1],\texttt{mem}[x])$. \Comment{Create $\frac{\partial J}{\partial \rmW_1}$.}
        \vspace{0.2em}
        \State  $\texttt{mem}[grad\_b_1] =f_{\text{mul}}(\texttt{mem}[\delta_1],\texttt{mem}[q])$. \Comment{Create $\frac{\partial J}{\partial \rvb_1}$.}
        \vspace{0.2em}
        \end{algorithmic}
    \end{algorithm}



==> transformer-large.tex <==
\def\usebigfont{1}
\input{main}
